A3Test: Assertion-Augmented Automated Test Case Generation

Test case generation is an important activity, yet a time-consuming and laborious task. Recently, AthenaTest -- a deep learning approach for generating unit test cases -- is proposed. However, AthenaTest can generate less than one-fifth of the test cases correctly, due to a lack of assertion knowledge and test signature verification. In this paper, we propose A3Test, a DL-based test case generation approach that is augmented by assertion knowledge with a mechanism to verify naming consistency and test signatures. A3Test leverages the domain adaptation principles where the goal is to adapt the existing knowledge from an assertion generation task to the test case generation task. We also introduce a verification approach to verify naming consistency and test signatures. Through an evaluation of 5,278 focal methods from the Defects4j dataset, we find that our A3Test (1) achieves 147% more correct test cases and 15% more method coverage, with a lower number of generated test cases than AthenaTest; (2) still outperforms the existing pre-trained models for the test case generation task; (3) contributes substantially to performance improvement via our own proposed assertion pre-training and the verification components; (4) is 97.2% much faster while being more accurate than AthenaTest.

==> architecture.tex <==
A Encoder stack: a stack of twelve layers of encoder blocks is implemented to derive the encoder hidden state used by the decoders. The encoder ~\cite{vaswani2017attention} encodes the input sequence of the focal method into a representation that can be used by the decoder. This representation would capture the structure and relationships between the elements of the method, such as variables, functions, and control flow statements.

Decoder: The decoder takes the encoded representation of the method as input and generate the test cases based on it. It uses the self-attention layers to capture the relationships between elements in the method and generate test cases that accurately test the method's functionality. The decoder generates the test cases token by token, using a combination of attention and fully connected layers. The layer normalization \cite{ba2016layer} component normalizes the input to each layer, which helps stabilize the training process and improve the model's ability to capture meaningful relationships between the elements in the input sequence of the method. The self-attention ~\cite{shaw2018self} component uses attention mechanisms it captures the relationships between elements in the method and generates test cases. The feed-forward component is a fully connected neural network that takes the output of the self-attention component as input and generates the final representation of the input sequence of the method.

Linear and Softmax: The linear and softmax components are used in the decoder to generate the test cases. The linear component transforms the final representation into a probability distribution over all possible test cases, while the softmax component normalizes these probabilities into a probability distribution with each iteration producing a more refined representation of the input sequence of the method. The final representation is then used by the decoder to generate the test cases. 


%\emph{A Encoder Stack} Each encoder block, like the original Transformer Encoder ~\cite{vaswani2017attention}, begins with a Layer Normalization ~\cite{ba2016layer} where the activation is only rescaled and no additive bias is applied ~\cite{raffel2020exploring}.  Each encoder block is made up of two parts: a multi-head self-attention layer with relative position encoding~\cite{shaw2018self} and a feed-forward neural network.  Each encoder's subcomponent has a residual connection around it, which is followed by a layer normalisation step~\cite{vaswani2017attention}. The self-attention mechanism [59]\kla{missing the citation} employs an information retrieval concept in which the relevant scores of each code token are computed using the dot product operation, with each token interacting with the other token only once. The self-attention mechanism is built around three major components: Query (Q), Key (K), and Value (V). The Query is a representation of the current code token that is used to score against all other tokens based on their keys, which are stored in the Key vectors. The attention scores of each token are calculated by taking the dot product of the Query and Key vectors. The attention weights are obtained by normalising the attention scores to probabilities using the Softmax function. 
% \kla{need tweaks a bit. looks like a copy and paste}
